Forward Compatible Training for Large-Scale Embedding Retrieval Systems

In visual retrieval systems, updating the embedding model requires recomputing features for every piece of data. This expensive process is referred to as backfilling. Recently, the idea of backward compatible training (BCT) was proposed. To avoid the cost of backfilling, BCT modifies training of the new model to make its representations compatible with those of the old model. However, BCT can significantly hinder the performance of the new model. In this work, we propose a new learning paradigm for representation learning: forward compatible training (FCT). In FCT, when the old model is trained, we also prepare for a future unknown version of the model. We propose learning side-information, an auxiliary feature for each sample which facilitates future updates of the model. To develop a powerful and flexible framework for model compatibility, we combine side-information with a forward transformation from old to new embeddings. Training of the new model is not modified, hence, its accuracy is not degraded. We demonstrate significant retrieval accuracy improvement compared to BCT for various datasets: ImageNet-1k (+18.1%), Places-365 (+5.4%), and VGG-Face2 (+8.3%). FCT obtains model compatibility when the new and old models are trained across different datasets, losses, and architectures.

==> FCT/sections/final_method.tex <==
\section{Method}\label{sec:method}

\subsection{Problem Setup}

A gallery set $\mathcal{G}$ is a collection of images, which are grouped into different clusters, $\{y_1\ldots y_n\}$. In visual retrieval, given a query image of a particular class, the goal is to retrieve images from $\mathcal{G}$ with the same class. A set of such query images is called the query set $\mathcal{Q}$. 

In embedding based retrieval, we have an embedding model $\phi: \mathbb{R}^{D}\to\mathbb{R}^{d}$ where $d << D$ and $D$ is the dimensionality of the input image, trained offline on some dataset $\mathcal{D}$ which is disjoint from $\mathcal{Q}$ and $\mathcal{G}$. Then, using some distance function $\mathfrak{D} : \mathbb{R}^d \times \mathbb{R}^d \to \mathbb{R}_{\geq 0}$, we get the closest possible image to query image $x_q\in\mathcal{Q}$ as $\argmin_{x\in\mathcal{G}} \mathfrak{D}(\phi(x_q), \phi(x))$. We use L2-distance for $\mathfrak{D}$ in our case. 

In our particular setup, we have two embedding models: the old model $\phi_{old}: \mathbb{R}^{D}\to\mathbb{R}^{d_{old}}$ and the new model $\phi_{new}: \mathbb{R}^{D}\to\mathbb{R}^{d_{new}}$, where $d_{old}, d_{new} << D$ are the embedding dimensions of old and new models, respectively. $\phi_{old}$ and $\phi_{new}$ are trained with datasets $\mathcal{D}_{old}$ and $\mathcal{D}_{new}$, respectively, using some supervised loss function.  

We assume $\phi_{old}$ is applied to every $x\in\mathcal{G}$, generating a collection of gallery embeddings, and  $\phi_{new}$ is applied to every $x_q\in\mathcal{Q}$, generating a set of query embeddings. Our goal is to design a method for performing retrieval between these two sets of embeddings without directly using the images in $\mathcal{G}$. We quantify the model compatibility performance as the accuracy of this retrieval.

% Consider two databases of images: (1) gallery-set () and (2) query-set (e.g. an image instance of one of these animals). These sets can be disjoint, overlapping, or the same. We assume we have features of all images in the gallery-set computed with $\phi_{old}$, and the features for the query-set images are obtained using $\phi_{new}$. Our goal is to recycle the features of the gallery-set images such that they become compatible with the features of query-set images. Hence, without using the original images from gallery-set we can re-use recycled features along with the new features.

% In this work we consider the standard supervised learning setup, however our framework is generalizable to other setups as well. We denote the old model as $\phi_{old}: \mathbb{R}^{D}\to\mathbb{R}^{d_{old}}$ and the new model as $\phi_{new}: \mathbb{R}^{D}\to\mathbb{R}^{d_{new}}$, where $D$ is the dimensionality of the input image and $d_{old}, d_{new} << D$ are the embedding dimensions of old and new models, respectively. $\phi_{old}$ and $\phi_{new}$ are trained with datasets $\mathcal{D}_{old}$ and $\mathcal{D}_{new}$, respectively, which are sets of image and label pairs $(x, y)$. The gallery-set $\mathcal{G}$ is disjoint from $\mathcal{D}_{old}$ and $\mathcal{D}_{new}$. For our experimentation, we also use the gallery-set also as the query-set $\mathcal{Q}$, however this is not required.\vivek{add implementation details section} 

\subsection{Forward Compatibility Setup}

In \fct{}, we define a function $\psi: \mathbb{R}^{D} \to \mathbb{R}^{d_{side}}$, which takes in an input from the $\mathcal{G}$ and produces our \info{}. Along with every embedding $\phi_{old}(x)$ for $x \in \mathcal{G}$ we also store the corresponding \info{} $\psi(x)$. Finally, we have a transformation model $h: \mathbb{R}^{d_{old}}\times \mathbb{R}^{d_{side}}\to\mathbb{R}^{d_{new}}$ which maps from $\phi_{old}$ and $\psi$ to $\phi_{new}$. In the \fct{} setup, we assume $\psi$ and $h$ are trained using $\mathcal{D}_{old}$ and  $\mathcal{D}_{new}$ training sets, respectively. To perform retrieval for $x_q\in\mathcal{Q}$ using $\psi$ and $h$, we take $\argmin_{x\in\mathcal{G}} \mathfrak{D}(\phi_{new}(x_q), h(\phi_{old}(x), \psi(x)))$. 
% Recent works \cite{meng2021learning,shen2020towards} approached the compatibility problem from perspective of making the new model compatible with the old model. We argue that this setup is overly restrictive. In most cases, we update the old model to a new one to reduce errors and/or remove bias. The compatibility objective (for example the influence loss in \cite{meng2021learning,shen2020towards}), on the other hand, encourage the new model to be similar to the old model. These are contradictory goals resulting in 1) less accurate/biased new model, and 2) poor compatibility performance.


\fct{} has a few key properties and constraints:


\noindent\textbf{1.} We do not modify the training of the new model, so it gets the highest possible accuracy.


\noindent\textbf{2.} We make the old model representation compatible to that of the new model through a learned transformation. 


\noindent\textbf{3.} As we discussed in the example of \autoref{fig:toy}, direct transformation from old embeddings to new may not be possible. When we train the old model, we \emph{prepare} for a future update by storing \info{} for each example in $\mathcal{G}$.
% We believe the compatibility problem cannot be solved after a model update
% The key idea in \fct{} is to store information at old time which might be useful at new time. Consider an extreme scenario, where a model is trained on a dataset with 100 classes and perfectly maps every input to the prototype embedding for each class. Now let's consider a more granular version of this dataset with a 1000 classes e.g. dogs are a class in the first dataset but in the second dataset are labeled with their individual breed. The old model will be invariant to dog breed, and therefore it will be impossible to learn a transfer function from old to new. Therefore, when we are computing the old embeddings, we should also compute discriminatory features which can help with future training. 

\vspace{2pt}\noindent\textbf{Efficiency} \fct{} comes with additional costs compared to BCT in computing side-information and updating. However, with a decentralized system design, we can mitigate these costs. See Appendix~\ref{sec:system} for more details on this decentralized design. Even without such a system, the computational cost of \fct{} is orders of magnitude lower than that of full backfilling (see Figure~\ref{fig:costs}). 

\begin{figure}[t]
\centering
    \includegraphics[width=0.7\columnwidth]{figures/transfer.pdf}
    \caption{\fct{} transformation model architecture and training. We use an MLP with BatchNorm~\cite{ioffe2015batch} for the projection layers and the mixer. The exact layer sizes are reported in Appendix~\ref{sec:hyperparams}.}\vspace{-10pt}
    \label{fig:transfer}
\end{figure}

\subsection{Training \fct{} Transformation} \label{sec:transformation}

For each sample $x\in\mathcal{D}_{new}$, we compute the transformation $h(\phi_{old}(x), \psi(x))$. Our objective to minimize is $\ell(x) = \|h(\phi_{old}(x), \psi(x)) - \phi_{new}\|_2^2$. In our case, we write $h$ as $h_\theta$, a neural network parameterized by $\theta$. Our final optimization problem can be written as $\theta^* = \argmin_{\theta} \sum_{x\in\mathcal{D}_{new}} \ell(x)$. The transformation model consists of two projection layers corresponding to old embedding and side-information branches followed by a mixing layer to reconstruct the new embedding (\autoref{fig:transfer}). We tested several alternative objectives, including KL divergence as in \cite{hinton2015distilling}, but found L2 loss to perform the best, in contrast to \cite{shen2020towards}, which finds that using L2 loss does not allow for backwards compatibility. Recently, \cite{budnik2021asymmetric} also observed superior performance using L2 loss between features for knowledge distillation. We provide training details in Section \ref{sec:hyperparams}.
%\subsection{Incorporating Side-Information} 



%To incorporate side information into our fused transfer model $h^s$, we introduce two learned projection functions: $p_s$ for the side-info and $p_t$ for the transfer function output. 

%\begin{equation}
%    h^s(x) = h(p_t(x), p_s(x))\label{eq:main-obj}
%\end{equation}

%where $h: (\mathbb{R}^d, \mathbb{R}^d)\to \mathbb{R}^d$. 
%the architectures for these transfer models are documented in Table \vivek{make table here} Section \ref{sec:analysis} shows an ablation on these projection functions. . We learn $h$, $p_t$ and $p_s$ jointly using the same objective as Equation~\label{eq:main-obj}

%We demonstrate a few possible versions of side-info, including central kernel alignment, ensemble side-info, and ensemble with mixup in Section~\ref{sec:results}. Note that in the \fct{} setup, we do not need access to the gallery set to train. However, we do require every example in the gallery set to be indexed with both an embedding vector and a piece of side-information.
\vspace{-1pt}
\subsection{Training \fct{} Side-Information}
% For a sample $x$, the best side-information is $\psi(x)=x$, as it contains all information about $x$ and hence works perfectly for reconstruction of new features. However, this is not a good choice since 1) it requires large storage and 2) large compute to reconstruct new features.  
The ideal side-information encodes compressed features for each example with which we can reconstruct new features given the old ones. This is a challenging task since we do not know about the future embedding model when learning the \info{}. The old model mainly learns features that are useful for its own training objective, and is (ideally) invariant to extraneous information. \textit{Side-information}, on the other hand, should be task independent, and capture features complementary to the old embeddings, that are useful for possible future updates.

Learning general features has been extensively studied in the context of unsupervised and contrastive learning \cite{chen2020simple,bachman2019learning,gidaris2018unsupervised,noroozi2016unsupervised,zhang2016colorful,doersch2015unsupervised} when labels are not available. Here, our objective is to learn task-independent features that are not necessarily relevant for the old task, and hence the labels. This makes unsupervised learning method a particularly interesting choice to learn \info{} for \fct{}. We use SimCLR contrastive learning \cite{chen2020simple} to train $\psi$. As a constraint of our setup, we can only train $\psi$ with data available at old training. We study other choices of side-information for \fct{} in Section~\ref{sec:side-info-ablate}. We provide details of the improved SimCLR training in the Appendix.


% We train $h$ with an L2 objective \vivek{do we need an equation header for something so simple} as follows
%The transfer function $h$ is a simple fully-connected neural network with batch-normalization \vivek{make table with architectures}. We train $h$ with an L2 objective \vivek{do we need an equation header for something so simple} as follows

%\begin{equation}
%    h = \argmin_h \sum_{(x, y) \in\mathcal{D}_{new}} \| h(\phi_{old}(x)) - %\phi_{new}(x)\|_2^2.
%\end{equation}


% Consider two versions of the model: v1 (old) and v2 (new). At v1-training, when we train $\phi_{old}$, we also train an \emph{encoder} model $g$ that maps each sample to a compressed side-information. We store $g(x) ~\forall x \in \mathcal{D}_g$. At v2-training we train $\phi_{new}$ independently. In addition we train a \emph{transformation} function $h$ that maps pairs of (old-feature, side-information) to new-features. Using $h$ we transform all old-features, making them compatible with the new features. Hence, for $x \in \mathcal{D}_q$ we compare $\phi_{new}(x)$ with $h( g(z), \phi_{old}(z))$ for all $z \in \mathcal{D}_g$. Note that in the \fct{} setup, we do not need to access the gallery-set, instead we use the old-features along with the side-information to recover the new-features. Besides, in \fct{} the new model is trained independently, and can have totally different learning setup (training data, optimization and loss, architecture, feature dimension, etc.) than the old model. The overall setup is shown in Figure \ref{fig:methods_comparison} (right). We show that this setup results in significant improvement compared to the BCT both when comparing new features against new features (i.e., the accuracy of the new model) and when comparing new feature with transformed old features (i.e., the compatibility accuracy). We explain how to obtain models $g$ and $h$ to satisfy compatibility in Section \ref{sec:gh}.
%------------------------------------------------------------------------

% \subsection{How to train \fct{} encoder and transformer?} \label{sec:gh}
% \begin{figure}[th]
%     \centering
%     \includegraphics[width=1.0\columnwidth]{figures/gh.pdf}
%     \caption{\fct{} encoder (left) and transformer (right) training.}
%     \label{fig:gh}
% \end{figure}
% The \fct{}-encoder, $g$, is trained on the old training-set to produce a compressed side-information per example. The side-information is meant to help transforming old features to new features. Essentially, given $\phi_{old}$ we are looking for a function $g$ such that $\forall \phi_{new} , \forall x \in \mathcal{D}_g$
% \begin{equation*}
% \exists h ~\text{ such that }~ h( g(x) , \phi_{old}(x)) = \phi_{new}(x)
% \end{equation*}
% With only the above constraint, $g(x) = x$ is a perfect solution. However, in practice we are looking for a side-information, $g(x)$, that is compressed. Hence, we limit to side-information to be the same size as the feature vector, i.e., $g(x) \in \mathbb{R}^d$.

% We train an auto-encoder on the old training set and use its encoder as $g$ as shown in Figure \ref{fig:gh} (left).


% The \fct{} transformer, $h$, is trained on the new training-set. The goal of $h$ is to recover new feature using the old feature and the side-information. We use a combination of multilayer perceptron (MLP) and side-net to train $h$ as shown in Figure \ref{fig:gh} (right).
% %------------------------------------------------------------------------


